CausalScore: An Automatic Reference-Free Metric for Assessing Response Relevance in Open-Domain Dialogue Systems

Automatically evaluating the quality of responses in open-domain dialogue systems is a challenging but crucial task. Current evaluation metrics often fail to align with human judgments, especially when assessing responses that are grammatically correct. To address this issue, we propose a novel metric, called CausalScore, which assesses the relevance of responses by measuring the causal strength between dialogue histories and responses. The causal strength is estimated by utilizing both unconditional dependence and conditional dependencies from the dialogue history to responses. We compare our metric with the existing competitive metrics in terms of their alignment with human judgements. Our experimental results demonstrate that CausalScore significantly surpasses existing state-of-the-art metrics by aligning better with human judgements. Additionally, we collect a new dialogue dataset CGDIALOG+ with human-annotated causal relations and a set of pairwise human judgements to facilitate the development of future automatic metrics.

==> sections/1_introduction_tao.tex <==
Relevance is an essential property in the development of open-domain dialogue systems that aspire to emulate human-like conversational abilities. Although the effectiveness of open-domain dialogue systems using large language models~\cite{zhang-etal-2020-dialogpt, ghazarian-etal-2021-discol, roller-etal-2021-recipes, 10.1145/3617829, feng-etal-2023-less, 10.1145/3604281}, replicating the nuanced relevance of human dialogue remains a challenge. Automatically measuring dialogue relevance for open-domain dialogue models persists as an open and under-investigated research problem, attributing to the one-to-many nature of dialogue~\cite{yeh-etal-2021-comprehensive, see-etal-2019-makes}.

Reference-based automatic metrics such as BLEU~\cite{papineni-etal-2002-bleu} and BERTScore~\cite{BERTScore}, assess dialogue responses by comparing semantic similarities with a standard "gold" response. However, the intrinsic nature of dialogues—that is, the potential for a single dialogue history to elicit a multitude of valid responses—renders these metrics inherently biased and misaligned with human judgment concerning relevance~\cite{liu-etal-2016-evaluate}. To overcome this issue,  reference-free metrics have been proposed, aiming to train a relevance scoring model by distinguishing human response and automatically generated negative responses, such as ADEM~\cite{lowe-etal-2017-towards}, RUBER~\cite{tao2018ruber}, and DEAM~\cite{ghazarian-etal-2022-deam}. However, these metrics tend to consider automatically generated responses as uniformly irrelevant, neglecting the varying degrees of relevance that occur in actual dialogues. \citet{huang-etal-2020-grade} have explored the use of topic transitions as a measure of relevance. While this approach captures certain aspects of dialogue dynamics, it fails to account for the full spectrum of semantics within utterances.

We suggest that the relevance of a response can be quantified by examining the causal relations between the dialogue history and the response. As illustrated in Figure~\ref{fig:causal_relation_example}, the human response receives the highest relevance score, attributed to the presence of three direct causes (\ie highlighted in yellow) within the dialogue history. The absence of any of these causes would render the human response baseless. In contrast, the response generated by \blenderbot is deemed relevant, albeit to a lesser extent than the human response, as it can be traced back to one immediate preceding question—"How much is the rent?". Meanwhile, the response from \constrain is rated with the least relevance due to its lack of any discernible causal relationship with prior utterances in history.

In this work, we introduce \ourmethod, an novel metric designed to automatically evaluate the relevance of responses. This metric is novel in its utilization of the strength of causal relations between the dialogue history and the response to compute a relevance score. By leveraging a simplified PC algorithm, \ourmethod can assess the causal strength from dialogue history to responses, and measure dialogue relevance that is more aligned with human judgements.

The implementation of \ourmethod involves a two-step process. Initially, we conduct (un)conditional independence tests using classification models to obtain causal relations, where classification models are trained in a supervised manner with human-annotated data. Subsequently, we quantify causal strength from dialogue history to response by using the probabilities of (un)conditional dependencies. Experimental results show that \ourmethod significantly outperforms other state-of-the-art dialogue metrics.

Our contributions are summarized as follows:
\begin{itemize}
    \item We propose \ourmethod, a novel automatic relevance metric for evaluating open-domain dialogue systems, which is the first attempt to introduce concepts of causal discovery into dialogue evaluation.
    \item We construct a new dialogue dataset CGDIALOG+ with 2444 human-annotated causal graphs, which expands upon the CGDIALOG dataset~\cite{feng-etal-2023-less}.
    \item We collect a new dataset of pairwise human judgements consisting of 1800 pairwise response assessments.
    \item We demonstrate the effectiveness of applying causal discovery to dialogue evaluation. The experiment results show that \ourmethod has significantly stronger correlations with human judgements than other state-of-the-art metrics.
\end{itemize}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/causal_relation_example.png}
    \caption{An illustrative example of a dialogue, with the corresponding responses generated by human and different dialogue systems. The human judgement score for relevance is provided alongside the outputs of the systems. \hl{Highlighted texts} indicate the causes of human response.}
    \label{fig:causal_relation_example}
\end{figure}

==> sections/2_method_tao.tex <==
In this paper, we propose an automatic evaluation metric, named \ourmethod, to assess the relevance of the corresponding responses to dialogue history. 
%
Formally, we are given a dialogue history $\vc=\{ c_1, ..., c_{t-1} \}$ and a response $r_t$, where each $c_i$ is an utterance in the history. The goal is to develop a function $f: (\vc, r_t) \rightarrow s$ that produces the relevance score $s$. We argue that \emph{a response exhibiting high relevance to the dialogue history inherently entails causal relations with the utterances in that dialogue history.} 

\reza{
To identify causal relations in dialogues, we propose a simplified PC algorithm using the classifier-based CI test. 
%In natural language, the same meaning can be expressed in various text forms. Thus, 
We assume there is a projection function $g(c_i)=\vz_i$, which maps an utterance to a \emph{continuous} latent random variable $\vz_i$ denoting the meaning of the utterance; the corresponding node in the causal graph is denoted by $v_i$. Utterances with similar meaning are thus mapped to the same latent  representation. 
%
%A causal graph in dialogue is directed acyclic graph $\gG=\{ \gV, \gE \}$, where a node represents a latent random variable $v_{\vz_i}$ and an edge represents a causal relation between a pair of nodes. 
                                                                %
For response evaluation, we only care about causal relations that involve responses. 
Thus, we can only focus on the causal relations between responses and dialogue history when running the simplified PC algorithm. 
 }

% In the original PC algorithm, the size of the conditioning set of independence tests increases iteratively from zero to $N-2$, where $N$ is the total number of random variables. In the simplified PC, to trade off the accuracy of causal discovery and computation efficiency, we limit the maximum size of the conditioning set to one. 

\ourmethod predicts a relevance score $s$ of a history-response pair $(\vc, r_t)$ in two steps: (1) running simplified PC algorithm to obtain causal relations between dialogue history $\vc$ and responses $r_t$, and (2) computing the relevance score based on the strength of causal relations.

\subsection{CGDIALOG+}
Our simplified PC algorithm needs classifier-based CI tests to identify causal relations. To conduct classifier-based CI tests, we need a dataset to train the  corresponding classifiers. CGDIALOG~\cite{feng-etal-2023-less} is a dialogue dataset with human-annotated causal graphs between dialogue history and responses. CGDIALOG randomly selected dialogues from the ESConv~\cite{liu-etal-2021-towards} and MSC~\cite{xu-etal-2022-beyond} datasets, and constructed 694 history-response pairs for ESConv and 800 history-response pairs for MSC. 
%
Due to the relatively small size of CGDIALOG, we extend it to CGDIALOG+ by adding 950 history-response pairs from the dialogues in DREAM~\cite{sun-etal-2019-dream}, following the same annotation instruction from \citet{feng-etal-2023-less}. In the first round of annotation, we hire four graduate computer science students to annotate causal graphs. Subsequently, in the second round, we require them to review each other's annotation outcomes to ensure consistency.  \reza{Reza: With how many annotators? Tao: More details in the preceding sentences.} We measure the inter-annotator agreement at both the utterance level and the clause level. At the utterance level, we compute Cohen's Kappa and obtain $0.8021$. At the clause level, we compute the averaged F1 score for all possible pairs of annotators and obtain an F1 score of $0.8316$. Both utterance and clause level scores indicate a high level of inter-annotator agreement. The statistics of CGDIALOG+ can be found in Table~\ref{tab:cgdialog_statistics}.

\input{tables/cgdialog_plus_statistics}

\subsection{Simplified PC Algorithm}

Our approach applies both conditional and unconditional independence tests, and is based on one assumption: \textit{if there is a causal relation between $c_i$ and $c_j$, and $i<j$, then $c_i$ is the cause and $c_j$ is the effect.} This  implies what interlocutors  said in the past influences what  they say in the future. 
%
This is in contrast to \constrain, proposed by 
\citet{feng-etal-2023-less}, which  makes three assumptions to reduce the computational complexity, leading to degradation in causal relations identification. 

In our simplified PC algorithm, we first conduct the \emph{unconditional} independence test to find utterances that have dependent relations with responses. Then, we apply the \emph{conditional} independence test. The conditional sets have a cardinality of one. 
%Sets with higher caridnality could  be considered too.  
There is less data to train  classifiers corresponding to higher cardinality sets for the CI test. Due to their unreliability and cost, we ignore the CI tests with larger conditional sets.

\paragraph{Unconditional Independence Classifier}
%First, we need to train a classifier for the unconditional independence test. 
To train this classifier, we need to build a data set in which positive examples are from $c^{+}_{i} \dep r_t$ (with  label $l=1$), and negative examples are from $c^{-}_{i} \indep r_t$ (with label $l=0$). \reza{Reza: Tao, is it correct? Tao: Yes}

As $c^{-}_{i} \indep r_t$ implies $c^{-}_{i}$ and $r_t$ are independent, we randomly sample utterances from other conversations as negative examples. 
%
We use $c_{t-1}$ as positive example, as they are often dependent to the responses.
%
This is supported by the study of \citet{feng-etal-2023-less}, which demonstrates that $90\%$ of preceding utterances serve as direct causes of the following responses. For the residual $10\%$ of preceding utterances that are not direct causes, they are highly likely to be statistically dependent on the responses. %The utilization of $c_{t-1}$ as positive examples is substantiated by empirical findings. 
We are thus able to establish a labeled training dataset comprising both positive and negative examples. The number of positive and negative examples within this dataset is equal. 

%denoted as $(c^{+}_{i}, r_t, 1)$, and negative examples, represented by $(c^{-}_{i}, r_t, 0)$. Furthermore, the quantity of positive and negative examples within this dataset is equal.

We use \roberta as the backbone model to develop the unconditional independence classifier. This is done by integrating a binary classification head, which is fed by the representation of the [CLS] token. \reza{As input to \roberta, we concatenate the context utterance $c_{i}$ with the response $r_t$ using the special token '</s>' as the delimiter. This amounts to the unconditional classifier $\mC_{uncond}$.
}

\paragraph{Conditional Independence Classifier}
Next, we need to train a classifier for the conditional independence test. To this end, it is imperative to construct a training set containing positive examples following $c^{+}_{i} \dep r_t | c_{k}$ and negative examples following $c^{-}_{i} \indep r_t | c_{k}$, where $c_{k}$ denotes an utterance that unconditionally depends on $r_t$. The previously established unconditional classifier $\mC_{uncond}$ determines the dependency relations between utterances and responses.

In order to construct this training set, we classify the annotated direct causes of responses in CGDIALOG+ as positive examples. In contrast, utterances that are not annotated as direct causes are designated as negative examples. The constructed dataset is denoted as $\sD_{L}$. We use the strategy of incremental self-training with constraints \cite{feng-etal-2023-less} to improve the performance of the conditional independence classifier. This method starts with the supervised training of an initial classifier $\mC_0$ on $\sD_{L}$. Then, $\mC_0$ is applied to unlabeled utterance tuples. Those tuples classified with a label of $1$ are incorporated into the training set as positive examples if they satisfy two criteria: 1) the probability $p(l=1| c_i, c_k, r_t)$ surpasses a predefined threshold $0.9$; 2) $c_i$ is $c_{t-2}$ or $c_{t-3}$. Then, a new classifier $\mC_1$ is trained on the updated training set $\sD^{0}$. The self-training cycle is repeated, each iteration yielding a new classifier $\mC_i$, until optimal performance is achieved on the validation set. The classifier ultimately chosen through this self-training process is denoted as $\mC_{cond}$.

\subsection{Compute Relevance Score}
Once we obtain the unconditional and conditional independence classifiers, we apply them to evaluate the relevance scores of responses. We compute causal strength from dialogue history to response (denoted as $\gS_{\vc\rightarrow r_t}$) to measure the relevance of responses. The total causal strength from dialogue history to responses is the sum of individual causal strength from utterance to response.
\begin{equation}
    \gS_{\vc\rightarrow r_t} = \sum_{c_i\in \vc} \gS_{c_i\rightarrow r_t}
\end{equation}

\citet{138734f0-eb1f-3daf-a1d4-a16462fb1be7, geiger2014estimating} shows causal strength between two variables, $\gS_{v_i\rightarrow v_j}$, can be measured by (C)MI $I(v_i; v_j)$ or $I(v_i;v_j|PA_{v_j}^{-v_i})$ in different causal graphs \footnote{\citet{138734f0-eb1f-3daf-a1d4-a16462fb1be7} shows $\gS_{v_i\rightarrow v_j}= I(v_i;v_j)$ or $\gS_{v_i\rightarrow v_j}\geq I(v_i;v_j|PA_{v_j}^{-v_i})$.}, where $PA_{v_j}^{-v_i}$ represent parents of $v_j$ excluding $v_i$. Considering the complexity of causal relations in dialogues, we employ both $I(v_i;v_j)$ and $I(v_i;v_j|PA_{v_j}^{-v_i})$ to measure causal strength. It makes sense because both $I(v_i;v_j)$ and $I(v_i;v_j|PA_{v_j}^{-v_i})$ measure strength of dependencies, and strength of dependencies imply causal strength~\cite{138734f0-eb1f-3daf-a1d4-a16462fb1be7}. However, it is still challenging to compute MI or CMI in the dialogue scenario. Considering the equivalent relation between CI test and CMI as we discussed in section~\ref{sec:background}, we use the probabilities of being dependent or conditional dependent produced by CI classifiers to measure causal strength.

Specifically, the unconditional independence classifier $\mC_{uncond}$ is applied to each pair of $(c_{i}, r_t)$, where $c_{i}$ represents individual utterances within the dialogue history. Then, we assess the unconditional dependence strength between each utterance and the response using probability $P(l=1 | c_i, r_t)$, where label 1 represents dependence. We denote this probability as $p_{+}(c_i,r_t)$ for simplicity. Then we collect utterances for which $p(c_i,r_t)$ exceeds 0.5 as unconditionally dependent utterances, denoted as $\gU_{c_i}^{dep}$.

Subsequently, the conditional classifier $\mC_{cond}$ is employed on tuples of the form $(c_i, c_j, r_t)$, where both $c_i$ and $c_j$ are elements of the set of unconditional dependent utterances $\gU_{uncond}$ and $i\neq j$. We then compute the probability of $P(l=1 | c_i, c_j, r_t)$ to assess the strength of conditional dependence between utterance and response, $p_{+}(c_i, c_j, r_t)$ for simplicity.

The scoring mechanism for \ourmethod considers both $p_{+}(c_i, r_t)$ and $p_{+}(c_i, c_j, r_t)$ as follows:
\begin{equation}
\begin{split}
    &\ourmethod(\vc, r_t) =\\
    &\frac{Avg(p_{+}(c_i,r_t)) + Avg(p_{+}(c_i, c_j, r_t))}{2}
\end{split}
\end{equation}
$c_i$ and $c_j$ are elements of the set $\gU_{c_i}^{dep}$, and the function $Avg$ indicates calculating the average of corresponding values. The score of \ourmethod ranges from 0 to 1, with higher values indicating better relevance.

==> tables/metric_corr_consistency.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Consistency}}     & \multicolumn{4}{c|}{\textbf{DREAM}}                                & \multicolumn{4}{c|}{\textbf{ESConv}}                               & \multicolumn{4}{c}{\textbf{MSC}}                                  \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}}  & \multicolumn{2}{c}{Voting}       & IgnoreEqual    & Cont2Cat       & \multicolumn{2}{c}{Voting}       & IgnoreEqual    & Cont2Cat       & \multicolumn{2}{c}{Voting}      & IgnoreEqual    & Cont2Cat       \\
\multicolumn{2}{c|}{}                         & Pearson        & Spearman        & Point-Biserial & IAA            & Pearson        & Spearman        & Point-Biserial & IAA            & Pearson        & Spearman       & Point-Biserial & IAA            \\ \hline
\multirow{5}{*}{Reference-based} & BLEU       & 0.045          & 0.050           & 0.041          & 0.225          & 0.049          & 0.009           & 0.014          & 0.241          & 0.047          & -0.007         & 0.015          & 0.216          \\
                                 & ROUGE      & 0.002          & -0.014          & -0.002         & 0.242          & -0.023         & -0.041          & -0.028         & 0.247          & 0.002          & -0.008         & -0.006         & 0.229          \\
                                 & METEOR     & -0.022         & -0.016          & -0.027         & 0.231          & 0.015          & 0.011           & 0.018          & 0.254          & -0.021         & -0.027         & -0.044         & 0.231          \\
                                 & BERTScore  & -0.001         & 0.012           & -0.003         & 0.228          & -0.036         & -0.033          & -0.042         & 0.258          & -0.005         & -0.015         & -0.009         & 0.229          \\
                                 & BLEURT     & 0.008          & 0.007           & 0.009          & 0.244          & -0.031         & -0.017          & -0.038         & 0.252          & -0.006         & -0.017         & -0.010         & 0.232          \\ \hline
\multirow{5}{*}{Reference-free} & PPL      & 0.014          &  0.025           & 0.012          & 0.260          & 0.017          & 0.011           & 0.020          & 0.270          & 0.012          & 0.027          & 0.053          & 0.275          \\ 
                                & GRADE      & 0.041          & 0.014           & 0.042          & 0.262          & 0.057          & 0.008           & 0.071          & 0.268          & 0.048          & 0.027          & 0.079          & 0.267          \\
                                 & DEAM       & 0.035          & 0.019           & 0.039          & 0.259          & 0.061          & 0.002           & 0.082          & 0.269          & 0.043          & 0.019          & 0.066          & 0.237          \\
                                 & ChatGPT    & 0.067          & 0.034           & 0.041          & 0.261          & 0.083          & 0.055           & 0.082          & 0.273          & 0.099          & 0.101          & 0.119          & 0.278          \\
                                 & GPT4       & 0.073          & 0.043           & 0.047          & 0.264          & 0.088          & 0.048           & 0.065          & 0.271          & 0.103          & 0.124          & 0.132          & 0.273          \\
                                 & \ourmethod & \textbf{0.206} & \textbf{0.234*} & \textbf{0.222} & \textbf{0.317} & \textbf{0.216} & \textbf{0.238*} & \textbf{0.287} & \textbf{0.337} & \textbf{0.214} & \textbf{0.231*} & \textbf{0.208} & \textbf{0.315} \\ \hline
\end{tabular}%
}
\caption{Correlations on \textbf{consistency} between automatic evaluation metrics and human judgements on three datasets.}
\label{tab:metric_corr_consistency}
\end{table*}

==> tables/metric_corr_empathy.tex <==

\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Empathy}}         & \multicolumn{4}{c|}{\textbf{DREAM}}                                  & \multicolumn{4}{c|}{\textbf{ESConv}}                                 & \multicolumn{4}{c}{\textbf{MSC}}                                     \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}}  & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       \\
\multicolumn{2}{c|}{}                         & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            \\ \hline
\multirow{5}{*}{Reference-based} & BLEU       & 0.019           & 0.058           & 0.012           & 0.225          & 0.069           & 0.050           & 0.024           & 0.205          & 0.019           & -0.020          & 0.007           & 0.203          \\
                                 & ROUGE      & 0.031           & 0.028           & 0.041           & 0.233          & 0.050           & 0.041           & 0.044           & 0.215          & 0.021           & 0.018           & 0.009           & 0.215          \\
                                 & METEOR     & 0.043           & 0.031           & 0.054           & 0.234          & 0.041           & 0.029           & 0.052           & 0.235          & 0.016           & 0.015           & 0.007           & 0.214          \\
                                 & BERTScore  & 0.065           & 0.077           & 0.103           & 0.238          & -0.028          & 0.004           & -0.035          & 0.238          & 0.032           & 0.042           & 0.052           & 0.220          \\
                                 & BLEURT     & 0.011           & 0.005           & 0.011           & 0.231          & 0.112           & 0.117           & 0.161           & 0.239          & 0.076           & 0.077           & 0.111           & 0.235          \\ \hline
\multirow{5}{*}{Reference-free} & PPL      & 0.018           & -0.031           & 0.016           & 0.242          & 0.021           & -0.018           & 0.008           & 0.245          & 0.030           & 0.032           & 0.061           & 0.248         \\ 
                                & GRADE      & 0.063           & 0.048           & 0.024           & 0.247          & 0.046           & 0.030           & 0.075           & 0.243          & 0.079           & 0.063           & 0.094           & 0.247          \\
                                 & DEAM       & 0.111           & 0.073           & 0.168           & 0.247          & 0.053           & 0.036           & 0.086           & 0.247          & 0.041           & 0.021           & 0.074           & 0.242          \\
                                 & ChatGPT    & 0.110           & 0.084           & 0.106           & 0.251          & 0.062           & 0.045           & 0.074           & 0.243          & 0.109           & 0.084           & 0.112           & 0.241          \\
                                 & GPT4       & 0.105           & 0.085           & 0.132           & 0.246          & 0.029           & 0.026           & 0.041           & 0.228          & 0.105           & 0.082           & 0.127           & 0.238          \\
                                 & \ourmethod & \textbf{0.131} & \textbf{0.252*} & \textbf{0.211} & \textbf{0.325} & \textbf{0.186} & \textbf{0.208*} & \textbf{0.302*} & \textbf{0.317} & \textbf{0.131} & \textbf{0.201} & \textbf{0.292*} & \textbf{0.314} \\ \hline
\end{tabular}%
}
\caption{Correlations on \textbf{empathy} between automatic evaluation metrics and human judgements on three datasets.}
\label{tab:metric_corr_empathy}
\end{table*}

==> tables/metric_corr_overall.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Overall}}         & \multicolumn{4}{c|}{\textbf{DREAM}}                                  & \multicolumn{4}{c|}{\textbf{ESConv}}                                 & \multicolumn{4}{c}{\textbf{MSC}}                                     \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}}  & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       \\
\multicolumn{2}{c|}{}                         & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            \\ \hline
\multirow{5}{*}{Reference-based} & BLEU       & 0.019           & 0.058           & 0.011           & 0.444          & 0.069           & 0.050           & 0.005           & 0.434          & 0.019           & -0.019          & 0.007           & 0.422          \\
                                 & ROUGE      & -0.031          & -0.028          & -0.040          & 0.453          & -0.030          & -0.041          & -0.044          & 0.445          & -0.011          & -0.018          & -0.010          & 0.435          \\
                                 & METEOR     & -0.043          & -0.031          & -0.053          & 0.454          & 0.041           & 0.029           & 0.052           & 0.455          & 0.006           & 0.015           & 0.007           & 0.435          \\
                                 & BERTScore  & 0.065           & 0.077           & 0.103           & 0.458          & -0.028          & 0.004           & -0.035          & 0.458          & 0.032           & 0.042           & 0.052           & 0.440          \\
                                 & BLEURT     & 0.011           & 0.005           & 0.011           & 0.451          & -0.112          & -0.117          & -0.161          & 0.439          & 0.076           & 0.077           & 0.112           & 0.445          \\ \hline
\multirow{5}{*}{Reference-free} & PPL      & 0.034           & 0.010           & 0.032           & 0.454          & 0.045           & 0.105           & 0.100           & 0.480          & 0.023           & -0.038           & -0.022           & 0.436          \\ 
                                & GRADE      & 0.054           & 0.033           & 0.012           & 0.454          & 0.023           & 0.011           & 0.004           & 0.436          & 0.088           & 0.050           & 0.105           & 0.442          \\
                                 & DEAM       & 0.111           & 0.107           & 0.168           & 0.467          & 0.013           & 0.010           & 0.005           & 0.442          & 0.042           & 0.021           & 0.074           & 0.442          \\
                                 & ChatGPT    & 0.153           & 0.101           & 0.113           & 0.460          & 0.052           & 0.055           & 0.041           & 0.463          & 0.129           & 0.125           & 0.181           & 0.481          \\
                                 & GPT4       & 0.159           & 0.157           & 0.141           & 0.486          & 0.048           & 0.062           & 0.042           & 0.471          & 0.131           & 0.103           & 0.119           & 0.486          \\
                                 & \ourmethod & \textbf{0.331*} & \textbf{0.422*} & \textbf{0.511*} & \textbf{0.595} & \textbf{0.287*} & \textbf{0.339*} & \textbf{0.411*} & \textbf{0.568} & \textbf{0.331*} & \textbf{0.401*} & \textbf{0.492*} & \textbf{0.569} \\ \hline
\end{tabular}%
}
\caption{Correlations on \textbf{overall} between automatic evaluation metrics and human judgements on three datasets.}
\label{tab:metric_corr_overall}
\end{table*}

==> tables/metric_corr_relevance.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Relevance}}       & \multicolumn{4}{c|}{\textbf{DREAM}}                                 & \multicolumn{4}{c|}{\textbf{ESConv}}                                & \multicolumn{4}{c}{\textbf{MSC}}                                    \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}}  & \multicolumn{2}{c}{Voting}        & IgnoreEqual    & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual    & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual    & Cont2Cat       \\
\multicolumn{2}{c|}{}                         & Pearson         & Spearman        & Point-Biserial & IAA            & Pearson         & Spearman        & Point-Biserial & IAA            & Pearson         & Spearman        & Point-Biserial & IAA            \\ \hline
\multirow{5}{*}{Reference-based} & BLEU       & 0.021           & 0.018           & 0.027          & 0.246          & -0.047          & -0.065          & -0.053         & 0.216          & 0.076           & 0.065           & 0.074          & 0.222          \\
                                 & ROUGE      & -0.005          & -0.008          & -0.015         & 0.272          & 0.039           & 0.020           & 0.045          & 0.243          & 0.091           & 0.087           & 0.090          & 0.249          \\
                                 & METEOR     & 0.028           & 0.033           & 0.043          & 0.262          & 0.097           & 0.097           & 0.081          & 0.243          & 0.013           & 0.036           & 0.087          & 0.241          \\
                                 & BERTScore  & -0.004          & -0.010          & -0.003         & 0.260          & 0.085           & 0.069           & 0.092          & 0.246          & 0.021           & 0.002           & 0.031          & 0.239          \\
                                 & BLEURT     & -0.022          & -0.032          & -0.030         & 0.257          & 0.025           & 0.022           & 0.026          & 0.246          & 0.074           & 0.089           & 0.094          & 0.249          \\ \hline
\multirow{5}{*}{Reference-free} & PPL      & 0.033           & 0.097          & 0.043          & 0.292          & -0.040           & -0.031           & -0.073          & 0.246          & -0.046          & -0.047           & -0.053          & 0.245          \\ 
                                & GRADE      & 0.004           & -0.005          & 0.035          & 0.248          & 0.013           & 0.021           & 0.030          & 0.248          & -0.003          & 0.012           & 0.049          & 0.243          \\
                                 & DEAM       & -0.090          & -0.053          & -0.121         & 0.273          & -0.011          & 0.039           & -0.011         & 0.257          & -0.012          & -0.032          & -0.007         & 0.253          \\
                                 & ChatGPT    & 0.036           & 0.024           & 0.088          & 0.284          & -0.002          & -0.018          & 0.096          & 0.250          & 0.083           & 0.084           & 0.109          & 0.271          \\
                                 & GPT4       & 0.049           & 0.038           & 0.083          & 0.263          & -0.002          & -0.023          & 0.097          & 0.251          & 0.039           & 0.083           & 0.110          & 0.277          \\
                                 & \ourmethod & \textbf{0.294*} & \textbf{0.334*} & \textbf{0.363} & \textbf{0.369} & \textbf{0.312*} & \textbf{0.343*} & \textbf{0.402} & \textbf{0.337} & \textbf{0.257*} & \textbf{0.308*} & \textbf{0.316} & \textbf{0.330} \\ \hline
\end{tabular}%
}
\caption{Correlations on \textbf{relevance} dimension between automatic evaluation metrics and human judgements on three different datasets (DREAM, ESConv, MSC). Inter-annotator agreement (IAA) is computed using Krippendorff's alpha. PPL represents perplexity. The asterisk * indicates results with p-value < 0.05, which are statistically significant.}
\label{tab:metric_corr_relevance}
\end{table*}

==> tables/metric_corr_specificity.tex <==
\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{ll|cccc|cccc|cccc}
\hline
\multicolumn{2}{c|}{\textbf{Specificity}}     & \multicolumn{4}{c|}{\textbf{DREAM}}                                  & \multicolumn{4}{c|}{\textbf{ESConv}}                                 & \multicolumn{4}{c}{\textbf{MSC}}                                     \\ \hline
\multicolumn{2}{c|}{\multirow{2}{*}{Metric}}  & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       & \multicolumn{2}{c}{Voting}        & IgnoreEqual     & Cont2Cat       \\
\multicolumn{2}{c|}{}                         & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            & Pearson         & Spearman        & Point-Biserial  & IAA            \\ \hline
\multirow{5}{*}{Reference-based} & BLEU       & -0.079          & -0.066          & 0.023           & 0.220          & 0.051           & 0.037           & 0.063           & 0.239          & 0.041           & 0.016           & 0.004           & 0.239          \\
                                 & ROUGE      & 0.043           & 0.052           & 0.049           & 0.259          & 0.046           & 0.043           & 0.061           & 0.253          & -0.001          & -0.019          & 0.001           & 0.251          \\
                                 & METEOR     & 0.066           & 0.061           & 0.081           & 0.251          & 0.093           & 0.040           & 0.080           & 0.259          & 0.002           & 0.011           & 0.001           & 0.263          \\
                                 & BERTScore  & 0.043           & 0.065           & 0.044           & 0.249          & 0.067           & 0.072           & 0.095           & 0.265          & 0.036           & 0.033           & 0.046           & 0.266          \\
                                 & BLEURT     & 0.041           & 0.038           & 0.050           & 0.249          & -0.003          & -0.004          & 0.003           & 0.258          & 0.031           & 0.020           & 0.046           & 0.261          \\ \hline
\multirow{5}{*}{Reference-free} & PPL      & 0.057           & 0.047           & 0.066           & 0.263          & -0.038           & 0.002           & -0.062           & 0.266          & -0.001           & -0.068           & -0.032           & 0.249          \\
                                & GRADE      & 0.047           & 0.031           & 0.058           & 0.251          & 0.057           & 0.047           & 0.071           & 0.271          & 0.063           & 0.041           & 0.069           & 0.268          \\
                                 & DEAM       & 0.063           & 0.029           & 0.078           & 0.255          & 0.039           & 0.015           & 0.059           & 0.274          & 0.048           & 0.039           & 0.047           & 0.253          \\
                                 & ChatGPT    & 0.026           & 0.017           & 0.033           & 0.266          & 0.042           & 0.039           & 0.054           & 0.276          & 0.070           & 0.082           & 0.085           & 0.286          \\
                                 & GPT4       & 0.057           & 0.038           & 0.057           & 0.260          & 0.017           & 0.014           & 0.016           & 0.258          & 0.069           & 0.068           & 0.080           & 0.263          \\
                                 & \ourmethod & \textbf{0.328*} & \textbf{0.434*} & \textbf{0.390*} & \textbf{0.360} & \textbf{0.324*} & \textbf{0.379*} & \textbf{0.411*} & \textbf{0.359} & \textbf{0.321*} & \textbf{0.356*} & \textbf{0.400*} & \textbf{0.355} \\ \hline
\end{tabular}%
}
\caption{Correlations on \textbf{specificity} between automatic evaluation metrics and human judgements on three  datasets.}
\label{tab:metric_corr_specificity}
\end{table*}
